Cicero: Addressing Algorithmic and Architectural Bottlenecks in Neural Rendering by Radiance Warping and Memory Optimizations

Neural Radiance Field (NeRF) is widely seen as an alternative to traditional physically-based rendering. However, NeRF has not yet seen its adoption in resource-limited mobile systems such as Virtual and Augmented Reality (VR/AR), because it is simply extremely slow. On a mobile Volta GPU, even the state-of-the-art NeRF models generally execute only at 0.8 FPS. We show that the main performance bottlenecks are both algorithmic and architectural. We introduce, CICERO, to tame both forms of inefficiencies. We first introduce two algorithms, one fundamentally reduces the amount of work any NeRF model has to execute, and the other eliminates irregular DRAM accesses. We then describe an on-chip data layout strategy that eliminates SRAM bank conflicts. A pure software implementation of CICERO offers an 8.0x speed-up and 7.9x energy saving over a mobile Volta GPU. When compared to a baseline with a dedicated DNN accelerator, our speed-up and energy reduction increase to 28.2x and 37.8x, respectively - all with minimal quality loss (less than 1.0 dB peak signal-to-noise ratio reduction).

==> coverpage.tex <==
\begin{titlepage} 

\twocolumn

\noindent\textbf{\large $\bigstar$ Major Changes:}
\begin{enumerate}
\item We revised \Sect{sec:algo:intuition} to show that high frame overlaps (computation reduction) are consistent across scenes and in real-world datasets. (\underline{Reviewer A})
\item We included new results (revised ``Datasets'' paragraph in \Sect{sec:exp}, updated \Fig{fig:real_scene_acc} and its texts in \Sect{sec:eval:acc}, and new \Sect{sec:eval:disc}) to show \proj's effectiveness and limitation on two real-world datasets. (\underline{Review A, C, E})
\item We added a new paragraph ``Broader Applicability'' at the end of \Sect{sec:mem:hw} to discuss how \proj’s hardware extensions can be applied beyond NeRF (\underline{Reviewer A})
\item We added a new paragraph ``SoC Integration'' in \Sect{sec:mem:hw} to argue that \proj hardware is agnostic to and integrates well with different GPUs. (\underline{Reviewer A})
\item We added a new \Sect{sec:back:basics} to discuss NeRF vs. traditional ray tracing (\underline{Reviewer B, D})
\item We revised the ``Warping-based Algorithms'' paragraph in \Sect{sec:related} to discuss our contribution compared to conventional image warping. (\underline{Reviewer B})
\item We added a new ``Memory Optimization in Rendering'' paragraph in \Sect{sec:related} to discuss our fully-streaming algorithm in the context of similar memory optimizations in ray tracing (\underline{Reviewer B})
\item We revised \Sect{sec:eval:comp} to clearly describe the baseline accelerator configurations to show that they are given equal or more compute resources (PEs) and on-chip memory sizes than our hardware (\underline{Reviewer B})
\item We revised the ``NeRF Algorithms'' paragraph in \Sect{sec:exp} to show that the NeRF models used for evaluation represent different memory-vs-speed trade-offs and to cover different feature representations. (\underline{Reviewer C})
\item We revised last paragraph in \Sect{sec:exp} to elaborate on offloading VR rendering to remote GPUs. (\underline{Reviewer D})
\item We revised \Sect{sec:algo:main} (penultimate paragraph) to show how we obtain the reference frame's pose, and added a footnote on Page 11 to discuss why we report a 3$\times$ speed-up for NeuRex but their paper reports  9$\times$. (\underline{Review E})
\item We revised \Sect{sec:mem:fs} to clarify 1) that our fully-streaming data flow does not incur storage overhead since the features are stored in memory \textit{as is} without reordering/duplication; what is being reordered is the order we \textit{access} the features, and 2) the Instant-NGP level at which we revert to the original data flow. (\underline{Review E})
\end{enumerate}

\noindent\textbf{\large $\bigstar$ Reviewer A}

\noindent\textbf{Previous work had pinpointed G as a bottleneck.}

Instant-3D~\cite{li2023instant} points to G as a bottleneck for a specific NeRF model InstantNGP and proposes a dedicated read mapper to handle the memory request. We identify two general bottlenecks in G, namely non-stream DRAM accesses and SRAM bank conflict with generally applicable solutions.  Improving these two general memory bottlenecks leads to a 28$\times$ improvement on average
%and, in particular, a 46$\times$ improvement on InstantNGP for G
(see \Fig{fig:gu_result}).

\noindent\textbf{Scheduling or compilation difficulties when moving to memory centric approach?}

The change of rendering order is taken care of by the GU, which simply iterates over the ray index table (\Fig{fig:hw_support} and \Sect{sec:mem:hw}) to issue memory accesses.

\noindent\textbf{Difficulties of integrating into PyTorch?}

No difficulty, as the evaluation is done using Pytorch.

\noindent\textbf{How’s NPU different from a standard TPU?}

No difference (first paragraph of \Sect{sec:exp}).  NPU is assumed to be part of the baseline SoC and is not our contribution.

\noindent\textbf{Area/power overhead of GPU, considering the added hardware components (e.g., GU and NPU)?}

No change to GPU hardware.
Our hardware extensions are limited to the NPU, which we consider as a part of the baseline mobile SoC (as with, e.g., Nvidia Xavier/Orin).
See \Fig{fig:arch}.

\noindent\textbf{Scalability w.r.t. GPU and rendering technologies.}

As rendering resolution increases, so do off-chip and on-chip pressure.  Our techniques to guarantee streaming DRAM access and eliminate bank conflicts are ever important.
\proj will benefit from recent progress in estimations of material properties; see the last paragraph of \Sect{sec:eval:disc}.
%~\cite{gkioulekas2013inverse, azinovic2019inverse}, based on which we can better interpolate, rather than simply warping, pixels between viewpoints across frames.

\noindent\textbf{Difference from DONeRF which uses ``spatial warping''?}

DONeRF and our method are \textit{completely} different and happen to use the same name (warping).  Our method reuses previously rendered pixels from reference frames to reduce work, while DONeRF ``\textit{warp[s] the entire space using a radial distortion, bringing the background closer to the view cell for positional encoding}''~\cite{neff2021donerf} without reusing previous pixels.

\noindent\textbf{Why incorporate max-pooling into NPU?}

To avoid extra data movements.  This is a common practice in today’s NPU design, e.g., Arm’s Ethos NPU~\cite{u55}.

%has a vector unit inside the NPU for operations like max-pooling (https://developer.arm.com/documentation/102420/latest/).

\noindent\textbf{Quantitative comparison with existing NeRF methods.}

In \Fig{fig:prior_work_comp} and \Sect{sec:eval:comp}, we compare our results against two existing NeRF accelerators (NeuRex and NGPC), and  achieve a speedup of 16.4$\times$ and 8.2$\times$, respectively.

\noindent\textbf{How does the fully-streaming NeRF rendering algorithm affect the accuracy and quality of rendering?}

\textit{No} accuracy loss, as only the computation \textit{order} is changed.

\noindent\textbf{Specific gains in relation to SRAM bank conflicts?}

We completely remove the bank conflict, leading to a 72.2$\times$ speed-up on feature gathering; see \Fig{fig:gu_result} and its texts.

\noindent\textbf{\large $\bigstar$ Reviewer D}

\noindent\textbf{Is it fair to compare a local rendering with a mobile Volta GPU with a discrete Turing GPU?}

No; they are two different real-world usage scenarios.
%Figure 19a shows our results in local rendering and Figure 19b shows our results in remote rendering.
The results are \textit{not} supposed to be compared against each other.

\noindent\textbf{\large $\bigstar$ Reviewer E}

%\textbf{Fully-streaming dataflow reorders vertex features and introduces storage overhead?}
%
%No storage overhead; the vertex features are stored in memory \textit{as is} without duplication.
%What is being reordered is the order we \textit{access} the features; see revision in \Sect{sec:mem:fs}.
%
%\textbf{At which Instant-NGP level do you revert to baseline?}
%
%Starting from level 5 (out of 8 levels); see revision in \Sect{sec:mem:fs}.

\noindent\textbf{Is using the reference frame via prediction provides more benefits than using previously rendered frames?}

Yes, and this is shown in \Fig{fig:acc}, where Temp-16 reuses a previously-rendered frame as a reference frame for 16 target frames.  Our Cicero-16 (which uses a predicted reference for 16 target frames) archives a 1-2 dB increase.

\noindent\textbf{Does the (ref/tgt) overlapping work for local rendering?}

In principle yes (a matter of engineering effort).
%, but they are just serialized in our current implementation.
Even without overlapping we still achieve 8.1$\times$ speedup (\Sect{sec:eval:perf}).

\noindent\textbf{Channel-major layout does not fully utilize on-chip bandwidth if feature size is less than the number of banks}

Yes; we address that by loading \textit{multiple} MVoxels batches.

\noindent\textbf{If 3D meshes exist, why render images via NeRFs?}

NeRF promises better rendering quality.  See \Sect{sec:back:basics}.

\end{titlepage}

